Hyperparameter-free Continuous Learning for Domain Classification in Natural Language Understanding

Domain classification is the fundamental task in natural language understanding (NLU), which often requires fast accommodation to new emerging domains. This constraint makes it impossible to retrain all previous domains, even if they are accessible to the new model. Most existing continual learning approaches suffer from low accuracy and performance fluctuation, especially when the distributions of old and new data are significantly different. In fact, the key real-world problem is not the absence of old data, but the inefficiency to retrain the model with the whole old dataset. Is it potential to utilize some old data to yield high accuracy and maintain stable performance, while at the same time, without introducing extra hyperparameters? In this paper, we proposed a hyperparameter-free continual learning model for text data that can stably produce high performance under various environments. Specifically, we utilize Fisher information to select exemplars that can "record" key information of the original model. Also, a novel scheme called dynamical weight consolidation is proposed to enable hyperparameter-free learning during the retrain process. Extensive experiments demonstrate that baselines suffer from fluctuated performance and therefore useless in practice. On the contrary, our proposed model CCFI significantly and consistently outperforms the best state-of-the-art method by up to 20% in average accuracy, and each component of CCFI contributes effectively to overall performance.

==> coverletter.tex <==
\section{Cover Letter }
\newcommand{\th}[1]{{\color{red}{(ting: #1)}}}
\newcommand{\yh}[1]{{\color{green}{(yh: #1)}}}


In the EMNLP review process, both Reviewer 1 and Reviewer 2 highly recommend our paper to be accepted. And all three reviewers agree that our paper has a comprehensive experimental evaluation. However, Reviewer 3 seems confused by some descriptions in our original EMNLP submission. In this cover letter, we address the comments of previous reviewers one by one. 

\subsection{Main concerns of Reviewer 3}
The main confusions of Reviewer 3 are as follows.
We marked the original comments as blue. 
\begin{enumerate}
    \item {\color{blue}{``There are (h x k) parameters in the model, so the Fisher information "matrix" has to be of shape (h x k) x (h x k)? In line 429, the Fisher information is defined as (h x k). Combined with equation (6), it seems like authors are only considering diagonal values of the Fisher information matrix.''}}
    
     There is clearly a misunderstanding here. The “Fisher information matrix” mentioned in our paper is different from the standard definition of Fisher information matrix. Ours is a matrix of the same dimension with weight matrix (h x k), while the standard definition of Fisher information matrix is a  square matrix. To avoid such confusion, we changed the “Fisher information matrix” into “parameter information table” in the new version, as shown in Step 3 of Section “Overall Process” (page 4). Each element is this table is the Fisher information of the corresponding parameter (to be precisely, the diagonal values of the standard Fisher information matrix). And therefore the size of the table is same with the number of retrainable parameters. 
     
     \item {\color{blue}{The proposed method seems to be a simple logistic regression classifier based on BERT features, and the complexity of the proposed method does not seem to be justified for such a simple model. Therefore, the paper's claim that the proposed method can accommodate more complex models such as neural networks doesn't seem to be correct. For linear models, there are more classic methods of summarizing data (for ex, leverage score based sampling, storing data points with nonzero dual parameters with SVM, etc). }}
     
     We thought Reviewer 3 had a misunderstanding here, since from our point of view, our model was definitely a neural network that can not be compared with SVM. Therefore, our rebuttal letter seems to be ``more confusing'' to Reviewer 3, as Reviewer 3 treats our model as “liner regression model” while we try to explain our model is a neural network.  In the final review, Reviewer 3 wrote this point as following:
{\color{blue}{``If parameters for the BERT are frozen and authors are only training the softmax layer, their model should still be a linear one.  ''}}
And we finally understand that Reviewer 3 means that our model is a BERT feature extractor plus a linear classifier, and he concerns whether our claim can still hold true for nonlinear classifiers.
Actually, our framework is a generic method that works for both linear and non-linear classifier. 
In this paper, most of our results are based on linear classifier (e.g., Figure 3 and 4), and we have some support experiments for the nonlinear classifier. In the last subsection of experimental evaluation “Fisher information sampling”, we use a two-layer dense model to examine the effectiveness of exemplars. Although the structure is simple, it is non-linear and therefore demonstrates that our proposed “Fisher information sampling” can be applied to the non-linear classifiers. 

\item {\color{blue}{``In line 223, authors suggest the classification task is the maximization of log probability, but the goal of classification should be maximizing the accuracy (or an appropriate metric for the task) rather than maximum likelihood estimation (MLE) itself being a goal? For machine learning, MLE is a mean to reach the goal. ''}}


 This is another misunderstanding of Reviewer 3. Our method is not related to MLE at all. To avoid this confusion, we have changed the description to improve the clarity.
 To be consistent with our other description, we keep the statement of ``maximize the probability'' in our problem definition, and  change some notations marked with $X$ to $D$, which includes both input examples ($X$) and labels ($Y$). 
\end{enumerate}

 

\subsection{Other questions of Reviewers}


\begin{enumerate}
\item {\color{blue}{(R3) What features does iCaRL use? Shouldn't they also be able to leverage BERT features? }}


 iCaRL is able to leverage BERT features, and in our implementation, iCaRL already uses BERT features,  as we mentioned in baselines of experimental section: ``To make fair comparisons, CCFI and all the baselines use the same BERT backbone.''   Original iCaRL uses CNN as its backbone, which is much worse than BERT in our evaluations. Therefore, to make a fair comparison, all baselines in our experiments are made to utilize BERT features.
 
 \item {\color{blue}{(R1) The proposed requires $O(n^2)$ space to store the fisher matrix, where n is the number of trainable parameters. When the trainable model is large (e.g., when the BERT model is fine-tuned), this method is almost inapplicable.}}
 
 Instead of $O(n^2)$ space, our method only requires $O(n)$ space to store the extra data structure (``parameter information table'' in the new version).
  And in most real-world applications of continual learning, only a small amount of retrainable parameters are needed to achieve comparative good performance. The initial input data usually contain a sufficient number of classes (e.g., in the factory, a product is trained with a large amount of data), while the  additional retrained data only contain a few new classes (e.g., when the product is bought by a user, she/he wants to add his/her own data of new classes). When the initial input data is  sufficiently large, it is safe to assume the first several layers are trained well enough to encode basic features from all existing and future domains. This observation is also confirmed by CoNDA (one of our comparison methods).  And that is why our proposed methodology is a combination of fixed feature extractor and tunable classifier.  Specifically, in our evaluation,  the size of  the Fisher information file (``parameter information table'' in the new version) is only 204KB on 73-domain data (performance shown in Figure 2) and 207KB on 150-class data (performance shown in Figure 3).  Compared to the size of BERT (usually 400MB+), the additional cost of storage space brought by our method is negligible. 

\end{enumerate}



		 	 	 		
			
				
					
						
					
				
			
		



\subsection{Summary of changes}

\begin{enumerate}
    \item We made minor changes to paraphrase some descriptions in introduction and method for improving the clarity. These small changes mainly target to address R3’s confusion.
  
  \item The changes in model description part are as follows:
    \begin{enumerate}
    \item As we describe above, the labels $Y$, the input $X$, and their union $D$, are defined more precisely. And we made correctness regarding the changes above,  throughout the model section. 
    \item We also add a subsection about the overall process to summarize the steps for both initial training and continual learning (retraining). 
%\item Change ``Fisher information matrix'' into  ``Parameter information table''.
%As mentioned multiple times above and in the paper, ``Parameter information table'' has the same amount of elements with trainable parameters, where each element is the Fisher information for the corresponding parameter.  
    \end{enumerate}
\end{enumerate}


